Generating Post-hoc Explanations for Skip-gram-based Node Embeddings by Identifying Important Nodes with Bridgeness

Node representation learning in a network is an important machine learning technique for encoding relational information in a continuous vector space while preserving the inherent properties and structures of the network. Recently, unsupervised node embedding methods such as DeepWalk, LINE, struc2vec, PTE, UserItem2vec, and RWJBG have emerged from the Skip-gram model and perform better performance in several downstream tasks such as node classification and link prediction than the existing relational models. However, providing post-hoc explanations of Skip-gram-based embeddings remains a challenging problem because of the lack of explanation methods and theoretical studies applicable for embeddings. In this paper, we first show that global explanations to the Skip-gram-based embeddings can be found by computing bridgeness under a spectral cluster-aware local perturbation. Moreover, a novel gradient-based explanation method, which we call GRAPH-wGD, is proposed that allows the top-q global explanations about learned graph embedding vectors more efficiently. Experiments show that the ranking of nodes by scores using GRAPH-wGD is highly correlated with true bridgeness scores. We also observe that the top-q node-level explanations selected by GRAPH-wGD have higher importance scores and produce more changes in class label prediction when perturbed, compared with the nodes selected by recent alternatives, using five real-world graphs.

==> background.tex <==
%!TEX root = main.tex



\section{Preliminary: DeepWalk and Euclidean Cut (EC)}

In this section, we first revisit the theoretical approximation of DeepWalk and definitions about Euclidean Cut (EC), which are proposed in previous work.

\begin{lemma}

(\cite{qiu2018network}). DeepWalk \cite{deepwalk} (thus, the special case of Node2Vec \cite{node2vec}) is equivalent to factorizing $\hat{M}=log(max(M,1))$ with

	\begin{equation}
		M=\frac{vol(A)}{T \cdot b}S, S=(\sum_{r=1}^T P^{r})D^{-1}, P=D^{-1}A,
	\end{equation}
where the embedding $Z^{*}$ is obtained by the singular value decomposition (SVD) of $\hat{M} = \hat{U} \hat{\Lambda} \hat{V}^T$ using the top-$k$ largest singular values / vectors, i.e., $Z^{*} = \hat{U}_{1:k} \hat{\Lambda}_{1:k}^{1/2}$,
\label{lemma:n2v}
\end{lemma}

Here $A$ is the adjacency matrix of an undirected and weighted graph $G$, and $V$ is a set of vertices in $G$. In addition, $D_{ii} = \sum_j A_{ij}$ is the diagonal degree matrix, $T$ is the window size, $b$ is the number of negative samples, and $vol(A) = \sum_{v_i,v_j \in V} A_{ij}$ is the volume. Using the Lemma \ref{lemma:n2v}, $Z^{*}$ could be used for the node embedding from the DeepWalk, and we explore its theoretical properties with respect to the change of found clusters from spectral clustering under edge perturbation. In particular, the quality of spectral clustering under perturbation is closely related to the change of eigenvectors of the Laplacian matrix (\cite{huang2009spectral}), and we focus on their theoretical properties in this paper.




Before analyzing the eigenvector $\hat{U}$, we first introduce \textit{Euclidean Cut (EC)} (\cite{bern1997approximation,ageev2014np,ageev2014complexity}). The \textit{Euclidean Cut (EC)} has been used for finding clusters by maximizing the \textit{EC} distance between clusters. The formal definition of the \textit{Euclidean Cut (EC)} is given in the below:
 
\begin{definition}
((Quadratic) Euclidean Cut (EC)) (\cite{ageev2014np}). Given a set $\mathcal{X}$ of points in $\mathbb{R}^k$, the (Quadratic) Euclidean Cut (EC) between two partitions, $\mathcal{N}$ and $\mathcal{\bar{N}}$ of the set $\mathcal{X}$, is defined as:\\
	\begin{equation}
		EC(\mathcal{N}, \mathcal{\bar{N}}|\mathcal{X}) = \sum_{i \in \mathcal{N}, j \in \mathcal{\bar{N}}} ||\mathcal{X}_{i,1:k} - \mathcal{X}_{j,1:k}||^2,
	\end{equation}
\end{definition}

Based on the definition above, we can generalize the distance metric to consider all clusters. In particular, when the euclidean space is given by a latent (eigenvector) space in $\hat{U}$, and the pair-wise distance could be computed accordingly. The new definition of \textit{Euclidean Cut (EC) in latent (eigenvector) space} is described as:

\begin{definition}
[Euclidean Cut (EC) in latent space] Assume that there is a set of clusters $C=\{C_1, C_2, ..., C_k\}$ from an input graph $G$ and $\hat{U}\in \mathcal{R}^{|V| \times k}$ is given from low-dimensional 
embeddings. The \textit{EC} in latent space is defined as:
	\begin{equation}
		\begin{aligned}
			EC(C_1, C_2, ..., C_k|\hat{U}) &= \sum_{m=1}^{k} EC(C_m, \bar{C}_m|\hat{U})\\
			&= \sum_{m=1}^{k} \sum_{v_i \in C_m, v_j\in \bar{C}_m} {|| \hat{U}_{i,1:k} - \hat{U}_{j, 1:k} ||^2}
		\end{aligned}		
	\end{equation}
\end{definition}


The distances above in the latent space can be normalized by the degree of each node to adjust the representation by its importance. For example, when the latent representations are from eigenvectors, the distance between degree-normalized eigenvectors is able to reflect their relative importance in the local scale and have been used for image segmentation (\cite{shi2000normalized}) and visualization (\cite{koren2003spectral}). The definition of degree-normalized \textit{DNEC} is given as:

\begin{definition}
[Degree-Normalized Euclidean Cut (DNEC) in latent space] Assume that there is a set of clusters $C=\{C_1, C_2, ..., C_k\}$ from an input graph $G$ and $\hat{U}\in \mathcal{R}^{|V| \times k}$ is given from low-dimensional 
embeddings (e.g., $Z^*$ in Lemma \ref{lemma:n2v}). The \textit{DNEC} in latent space is defined as:
	\begin{equation}
			DNEC(C_1, C_2, ..., C_k|\hat{U},D) = \sum_{m=1}^{k} \sum_{v_i \in C_m, v_j\in \bar{C}_m} {|| \frac{\hat{U}_{i,1:k}}{d_i} - \frac{\hat{U}_{j, 1:k}}{d_j} ||^2},
	\end{equation}
\end{definition}
where $D$ is the degree matrix of an input graph $G$.

